Conceptual Mapping of Controversies

With our work, we contribute towards a qualitative analysis of the discourse on controversies in online news media. For this, we employ Formal Concept Analysis and the economics of conventions to derive conceptual controversy maps. In our experiments, we analyze two maps from different news journals with methods from ordinal data science. We show how these methods can be used to assess the diversity, complexity and potential bias of controversies. In addition to that, we discuss how the diagrams of concept lattices can be used to navigate between news articles.

==> tikzlibraryfca.code.tex <==
%%
%% This is file `tikzlibraryfca.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% latex-fca.dtx  (with options: `tikz,package')
%%  latex-fca.dtx
%%  Copyright ℂ 2022 Ernst-Schröder-Zentrum
%%                   für Begriffliche Wissensverarbeitung
%%  Authors: Bernhard Ganter
%%           Tobias Schlemmer
%% 
%%  This program is provided under the terms of the
%%  LaTeX Project Public License distributed from CTAN
%%  archives in directory macros/latex/base/lppl.txt.
%% 
%%  This work is "maintained" (as per LPPL maintenance status) by
%%  Tobias Schlemmer <keinstein@users.sf.net>.
%% 
%%  This work consists of the files
%%    latex-fca.dtx and
%%    latex-fca.ins
%% 
%%  and the derived files
%%    fca.sty,
%%    formula0.cxt,
%%    formula1.cxt.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesFile{tikzlibraryfca.code.tex}
    [2022/09/17 v3.0
 TikZ support for Formal Concept Analysis]
\RequirePackage{fca}
\let\fca@tikz@without@library\relax
\def\fca@generate@tikz@parameter#1#2#3{%
  \pgfkeysdef{/fca/#1}{\pgfkeys{/tikz/#1=##1}}
  \pgfkeyssetvalue{/fca/#1}{#3}%
}
\@ifpackagelater{tikz}{2020/09/28}{}{%
  \PackageWarning{fca}{Your TikZ version does not fully support fca
    name spaces.^^J
    I'm trying to fix that..., trying to apply^^J
    patch 88951be592b558b94b14a97aaffe9df6c1ce61ee from TikZ}
  \def\tikz@calc@anchor#1.#2\tikz@stop{%
    % Check if a shape with name prefix exists, otherwise try the global name
    % without prefix.
    \ifcsname pgf@sh@ns@\tikz@pp@name{#1}\endcsname%
      \pgfpointanchor{\tikz@pp@name{#1}}{#2}%
    \else
      \pgfpointanchor{#1}{#2}%
    \fi
  }%
\def\tikz@subpicture@handle@#1{
  \pgfkeys{/tikz/pics/.cd,#1}%
  \tikz@node@transformations%
  \let\tikz@transform=\relax%
  \let\tikz@picmode\tikz@mode%
  \tikzset{name prefix ../.style/.expanded={/tikz/name prefix=\pgfkeysvalueof{/tikz/name prefix}}}%
  \ifx\tikz@fig@name\pgfutil@empty\else%
    \tikzset{name prefix/.expanded=\tikz@fig@name}%
  \fi%
  \pgfkeysvalueof{/tikz/pics/setup code}%
  \pgfkeysgetvalue{/tikz/pics/code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@whichbox=\hbox\bgroup%
    \unhbox\tikz@whichbox%
      \hbox\bgroup
      \bgroup%
      \pgfinterruptpath%
      \pgfscope%
      \tikz@options%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \tikz@atbegin@scope%
      \scope[every pic/.try]%
      \tikz@pic@code%
      \endscope%
      \tikz@atend@scope%
      \endpgfscope%
      \endpgfinterruptpath%
      \egroup
      \egroup%
      \egroup%
    \fi%
    \pgfkeysgetvalue{/tikz/pics/foreground code}{\tikz@pic@code}
    \ifx\tikz@pic@code\pgfutil@empty\else%
      \setbox\tikz@figbox=\hbox\bgroup%
      \unhbox\tikz@figbox%
      \hbox\bgroup
      \bgroup%
      \pgfinterruptpath%
      \pgfscope%
      \tikz@options%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \tikz@atbegin@scope%
      \scope[every front pic/.try]%
      \tikz@pic@code%
      \endscope%
      \tikz@atend@scope%
      \endpgfscope%
      \endpgfinterruptpath%
      \egroup
      \egroup%
      \egroup%
    \fi%
    \pgfkeysgetvalue{/tikz/pics/background code}{\tikz@pic@code}
    \ifx\tikz@pic@code\pgfutil@empty\else%
      \setbox\tikz@figbox@bg=\hbox\bgroup%
      \unhbox\tikz@figbox@bg%
      \hbox\bgroup
      \bgroup%
      \pgfinterruptpath%
      \pgfscope%
      \tikz@options%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \tikz@atbegin@scope%
      \scope[every behind pic/.try]%
      \tikz@pic@code%
      \endscope%
      \tikz@atend@scope%
      \endpgfscope%
      \endpgfinterruptpath%
      \egroup
      \egroup%
      \egroup%
    \fi%
    \tikz@node@finish%
  }%
\def\tikz@parse@node#1(#2){%
  \pgfutil@in@.{#2}% Ok, flag this
  \ifpgfutil@in@
    \tikz@calc@anchor#2\tikz@stop%
  \else%
    \tikz@calc@anchor#2.center\tikz@stop% to be on the save side, in
                                % case iftikz@shapeborder is ignored...
    \ifcsname pgf@sh@ns@\tikz@pp@name{#2}\endcsname
      \expandafter\ifx\csname pgf@sh@ns@\tikz@pp@name{#2}\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{\tikz@pp@name{#2}}%
      \fi%
    \else\ifcsname pgf@sh@ns@#2\endcsname
      \expandafter\ifx\csname pgf@sh@ns@#2\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{#2}%
      \fi%
    \fi\fi
  \fi%
  \edef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}%
 }%
\fca@generate@tikz@parameters
\@for \@tempa:=%
shape,
text ragged,%
text badly ragged,%
text ragged left,%
text badly ragged left,%
text justified,%
text centered,%
text badly centered,%
even odd rule,%
nonzero rule,%
fill opacity,%
opacity,%
blend mode,%
color,%
rotate,%
solid,%
dotted,%
loosely dotted,%
densely dotted,%
line width,%
x,%
y%
\do {
  \edef\@tempb{%
    \noexpand\pgfkeysdef{/fca/\@tempa}{\noexpand\pgfqkeys{/tikz}{\@tempa={##1}}}%
  }%
  \@tempb
}
\pgfkeysdef{/fca/options}{\tikz@addoption{#1}}
\pgfkeysdef{/fca/stroke}{%
  \pgfqkeys{/tikz}{draw={#1}}%
  \fca@testoption{#1}{%
    \fca@append\fca@usepath{stroke,}%
  }{}{%
    \fca@append\fca@usepath{stroke,}%
  }%
}
\pgfkeysdef{/fca/fill}{%
  \pgfqkeys{/tikz}{fill={#1}}%
  \fca@testoption{#1}{%
    \fca@append\fca@usepath{fill,}%
  }{}{%
    \fca@append\fca@usepath{fill,}%
  }%
}
\def\fca@options{\tikz@options}%
\def\fca@defaultoptions{\tikz@options}%
\def\fca@transform{\tikz@transform}%
\@ifundefined{tikz@transform}{\let\tikz@transform\empty}{}
\let\fca@ifintikz\@secondoftwo
\tikzaddtikzonlycommandshortcutlet\fca@ifintikz\@firstoftwo
\fcaset{%
  attributes left/.append style={
    align=flush right
  },
  attributes center/.append style={
    align=flush center
  },
  attributes right/.append style={
    align=flush left
  },
  objects left/.append style={
    align=flush right
  },
  objects center/.append style={
    align=flush center
  },
  objects right/.append style={
    align=flush left
  }
}

\let\fca@notikz@parse@paren@vector\fca@parse@paren@vector
\newcommand\fca@tikz@parse@paren@vector[3]{%
  \def\tikz@coordinate@caller{%
    \fca@notikz@parse@paren@vector{#1}{#2}{#3}%
  }%
  \tikz@scan@one@point \tikz@@coordinate@at@math
}

\newcommand\fca@tikz@oldnode[4]{%
  \begin{pgfscope}%
    \fca@nodeslayer
    \path (#3,#4) node[
      anchor=center,
      shape=circle,
      /fca/.cd,
      /fca/every node/.try,
      /fca/every concept/.try,
      #1]
      (#2) {} ;%
      \fca@endnodeslayer
    \iffca@draft
      \ifthenelse{\boolean{fca@CircledNumbers}}{%
        \fca@nodenumberslayer
        \path[overlay] (#2)
        node[
        shape=circle,
        anchor=center,
        /fca/.cd,
        /fca/every node/.try,
        /fca/every concept/.try,
        #1
        /fca/.cd,
        /fca/node number,
        draw=none]%
        (#2 number)
        {#2};%
        \fca@endnodenumberslayer
      }{}%
    \fi
  \end{pgfscope}%
  \ignorespaces
}
\newcommand{\fca@tikz@oldedge}[3]{%
  \fca@edgeslayer
  \path[draw,/fca/.cd,every edge/.try,#1] (#2) edge (#3);%
  \fca@endedgeslayer
  \ignorespaces
}

\newcommand\fca@tikz@labelBox[1]{%
  \begin{scope}%
    \fcaset{every node/.try,every label/.try,#1}%
    \edef\@tempa{\pgfkeysvalueof{/fca/pgfnode}}%
    \xdef\fca@temp@node@name{%
      \expandafter\fca@remove@anchor\expandafter{\@tempa}%
    }%
    \fca@labelslayer
      \path[/fca/.cd,every node/.try,every label/.try,#1]
      (\fca@temp@node@name.\fca@label@at)
      ++(\fca@label@shift@x,\fca@label@shift@y)
      node[shape=rectangle] (%
        \pgfkeysvalueof{/fca/label/name prefix}%
        \pgfkeysvalueof{/fca/node}%
        \pgfkeysvalueof{/fca/label/name suffix}%
      ){%
        \pgfkeysvalueof{/fca/node contents}%
      };%
    \fca@endlabelslayer
    \iffca@connectors
      \begin{scope}
        \fca@connectorslayer
        \path[draw,/fca/.cd,#1,every label edge/.try,/tikz/.cd]
        (\pgfkeysvalueof{/fca/node}) --
        (%
        \pgfkeysvalueof{/fca/label/name prefix}%
        \pgfkeysvalueof{/fca/node}%
        \pgfkeysvalueof{/fca/label/name suffix}%
        .\pgfkeysvalueof{/fca/anchor}) ;
        \fca@endconnectorslayer
      \end{scope}%
    \fi
    \begin{scope}
      \fcaset{shape=coordinate,#1}%
      \fcaset{%
        every label concept/.try}%
      \fcaset{%
        label concept/.try
      }%
      \def\@tempa{coordinate}%
      \ifx\@tempa\tikz@shape
      \else
        \fca@labelconceptslayer
        %\edef\fca@tempa{
        \path
          (\fca@temp@node@name.\fca@label@at)%
          node[draw,
          /fca/.cd,
          shape=coordinate,
          #1,
          every label concept/.try,
          label concept/.try]
        (\pgfkeysvalueof{/fca/label/name prefix}%
          \pgfkeysvalueof{/fca/node}%
          \pgfkeysvalueof{/fca/label/name suffix}%
          ){};
        % \pgfsetstrokecolor{\fca@node@color}%
        %\pgfnode{}{\pgfkeysvalueof{/fca/anchor}}{}{}%
        \fca@endlabelconceptslayer
      \fi
    \end{scope}
  \end{scope}%
  \ignorespaces
}
\newcommand\fca@tikz@startdiagram[1][]{%
  \fca@notikz@startdiagram%
  \fca@tikz@diagram@
}
\newcommand\fca@tikz@Defaults{
  \fca@notikz@Defaults
  \pgfkeysgetvalue{/tikz/name prefix}{\fca@tikz@origprefix}%
  \pgfkeysgetvalue{/fca/name prefix}{\@tempb}%
  \let\@tempa\fca@tikz@origprefix
  \fca@concat\@tempa\@tempb%
  \pgfqkeys{/tikz}{%
    name prefix/.expand once=\@tempa
  }%
  \pgfkeysgetvalue{/fca/name suffix}{\@tempa}%
  \pgfkeysgetvalue{/tikz/name suffix}{\@fca@tikz@origsuffix}%
  \fca@concat\@tempa\@fca@tikz@origsuffix%
  \pgfqkeys{/tikz}{%
    name suffix/.expand once=\@tempa
  }%
  \pgfkeyssetvalue{/fca/name prefix}{%
    \pgfkeysvalueof{/tikz/name prefix}%
  }%
  \pgfkeyssetvalue{/fca/name suffix}{%
    \pgfkeysvalueof{/tikz/name suffix}%
  }%
}
\tikzaddtikzonlycommandshortcutlet\fca@oldnode\fca@tikz@oldnode
\tikzaddtikzonlycommandshortcutlet\fca@oldedge\fca@tikz@oldedge
\tikzaddtikzonlycommandshortcutlet\fca@@labelBox\fca@tikz@labelBox
\tikzaddtikzonlycommandshortcutlet\fca@parse@paren@vector\fca@tikz@parse@paren@vector
\tikzaddtikzonlycommandshortcutlet\fca@notikz@Defaults\fca@Defaults
\tikzaddtikzonlycommandshortcutlet\fca@Defaults\fca@tikz@Defaults
\newenvironment{tikzdiagram}[1][]{%
  \def\fca@begindiagram{%
    \begin{tikzpicture}%
      \fcaset{#1}%
      \unitlength=\dimexpr\pgf@xx+\pgf@yx\relax
    }%
    \noindent
    \@ifnextchar\bgroup\fca@olddiagram\fca@diagram% This line must be
    % executed before \begin{pgfpicture}
  }{%
  \end{tikzpicture}%
}
\fcaset{copy unitlength/.style={%
    x=\unitlength,
    y=\unitlength,
  }
}
\endinput
%%
%% End of file `tikzlibraryfca.code.tex'.

